How to Refactor this Code? An Exploratory Study on Developer-ChatGPT Refactoring Conversations

Large Language Models (LLMs), like ChatGPT, have gained widespread popularity and usage in various software engineering tasks, including refactoring, testing, code review, and program comprehension. Despite recent studies delving into refactoring documentation in commit messages, issues, and code review, little is known about how developers articulate their refactoring needs when interacting with ChatGPT. In this paper, our goal is to explore conversations between developers and ChatGPT related to refactoring to better understand how developers identify areas for improvement in code and how ChatGPT addresses developers' needs. Our approach relies on text mining refactoring-related conversations from 17,913 ChatGPT prompts and responses, and investigating developers' explicit refactoring intention. Our results reveal that (1) developer-ChatGPT conversations commonly involve generic and specific terms/phrases; (2) developers often make generic refactoring requests, while ChatGPT typically includes the refactoring intention; and (3) various learning settings when prompting ChatGPT in the context of refactoring. We envision that our findings contribute to a broader understanding of the collaboration between developers and AI models, in the context of code refactoring, with implications for model improvement, tool development, and best practices in software engineering.

==> Sections/06_Threats.tex <==
%\vspace{-.2cm}
\section{Threats To Validity}
\label{Section:Threats}

The first threat relates to the analysis of open-source projects. Although our dataset covers different programming languages, our results may not generalize to systems written in other languages that are not considered in this study. %Another potential threat to validity relates to our findings regarding counting the reported quality attributes and code smells. Due to the large number of issues associated with refactorings, we have not performed a manual validation to remove false positive issues. Thus, this may have an impact on our findings. 
Further, we constructed our dataset by extracting data source types that contain the term `refactor' in the prompt. There is the possibility that we may have excluded synonymous terms/phrases. However, even though this approach reduces the number of source types in our dataset, it also decreases false-positives, and ensures that we analyze artifacts that are explicitly focused on refactorings.


==> Tables/Project_Overview.tex <==
\begin{table}[h!]
\begin{center}
\caption{Summary of the extracted data.}
\label{Table:DATA_Overview}
%\begin{adjustbox}{width=0.32\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lllll}\hline
\toprule
\bfseries Item & \bfseries Count \\
\midrule
%ChatGPT Prompt having keyword `\textit{refactor*}' &  \\
Refactoring GitHub commits & 470 \\
Refactoring GitHub issues & 69 \\
Refactoring GitHub code files & 176 \\
%Refactoring Hacker News &  \\
\bottomrule
\end{tabular}
%\end{adjustbox}
\end{center}
\vspace{-.5cm}
\end{table}
